Triangulated Surface Denoising using High Order Regularization with Dynamic Weights

Recovering high quality surfaces from noisy triangulated surfaces is a fundamental important problem in geometry processing. Sharp features including edges and corners can not be well preserved in most existing denoising methods except the recent total variation (TV) and $\ell_0$ regularization methods. However, these two methods have suffered producing staircase artifacts in smooth regions. In this paper, we first introduce a second order regularization method for restoring a surface normal vector field, and then propose a new vertex updating scheme to recover the desired surface according to the restored surface normal field. The proposed model can preserve sharp features and simultaneously suppress the staircase effects in smooth regions which overcomes the drawback of the first order models. In addition, the new vertex updating scheme can prevent ambiguities introduced in existing vertex updating methods. Numerically, the proposed high order model is solved by the augmented Lagrangian method with a dynamic weighting strategy. Intensive numerical experiments on a variety of surfaces demonstrate the superiority of our method by visually and quantitatively.

==> Algorithm.tex <==

%Assume $f \in V_M$, $u \in V_{M}$, the total variation model (ROF) aims at solving
%
%\begin{equation*}
% \min \limits_{u\in V_M}\{E_{\mathrm{tv}}(u) =R_{\mathrm{tv}}(\nabla_{M}u)+\frac{\alpha}{2}\left\| u-f \right\|^2_{V_M}\},
%\end{equation*}
%where $R_{\mathrm{tv}}$ is the total variation of $u$ and $\alpha$ is a positive fidelity parameter.





%\subsection{Mesh Denoising Algorithm}
%Base on the augmented Lagrangian method, we present an iterative mesh denoising algorithm, with high order total variation normal filtering model and vertex update model introduced in subsection \ref{sec:HOTVModel} and \ref{sec:VertexUpdateModel} respectively, which is described in Algorithm \ref{alg:MeshDenoising}.
%
%\begin{algorithm}
%\caption{Augmented Lagrangian method for mesh denoising} %$(B_i = \{C_i, Q_i, T_i, E_i\})$}
%\label{alg:MeshDenoising}
%\textbf{Initialization:} $i=0$, $I = 3$, $\epsilon_V = 1e-3$.
%
%    \textbf{Repeat}
%        \begin{itemize}
%          \item [1.] Normal filtering using high order total variation model \eqref{InitHOTVmodel};
%
%          \textbf{Initialization:} $\lambda^{0}=0, \mathbf{p}^{-1}=0, \mathbf{N}^{-1}=0, k=-1, K=100, \epsilon_N = 1e-4;$
%
%          \textbf{Repeat}
%          \begin{itemize}
%            \item[1.1] $\mathbf{N}$-sub problem
%
%            For fixed $(\lambda^k, \mathbf{p}^{k-1})$ solve three sparse linear system by \eqref{eqn:n-sub1};
%
%            Normalize $\mathbf{N}^k$;
%
%            \item[1.2] $\mathbf{p}$-sub problem
%
%            For fixed $(\lambda^k, \mathbf{N}^k)$ compute $\mathbf{p}$ by \eqref{eqn:p-closedSolution};
%
%            Compute $w_l$ by using \eqref{eqn:weightFunction};
%
%            \item[1.3] Update Lagrange multipliers
%
%            $\lambda^{k+1} = \lambda^{k} + r(\mathbf{p}^k - \nabla^2 \mathbf{N}^k)$;
%
%          \end{itemize}
%          \textbf{Until} ($ \|\mathbf{N}^k - \mathbf{N}^{k-1}\|^2_{V_M}< \epsilon_N$ or $k \geq K$)
%
%          \item [2.] Update vertex positions using the vertex updating model \eqref{eq:Sun};
%
%          \item [3.] Get new face normal field $\mathbf{N}^{'}$ from updated vertices;
%
%        \end{itemize}
%    \textbf{Until} ($ \|\mathbf{N}^k - \mathbf{N}^{'}\|^2_{V_M}< \epsilon_V$ or $i \geq I$)
%%\quad \ \  \textbf{Return} narrow band data structure $B_i = \{C_i, Q_i, T_i, E_i\}$.
%\end{algorithm}

%\noindent \textbf{\textit{remark}} xxxxxxxxxxx

